Regret Circuits: Composability of Regret Minimizers

Regret minimization is a powerful tool for solving large-scale problems; it was recently used in breakthrough results for large-scale extensive-form game solving. This was achieved by composing simplex regret minimizers into an overall regret-minimization framework for extensive-form game strategy spaces. In this paper we study the general composability of regret minimizers. We derive a calculus for constructing regret minimizers for composite convex sets that are obtained from convexity-preserving operations on simpler convex sets. We show that local regret minimizers for the simpler sets can be combined with additional regret minimizers into an aggregate regret minimizer for the composite set. As one application, we show that the CFR framework can be constructed easily from our framework. We also show ways to include curtailing (constraining) operations into our framework. For one, they enables the construction of CFR generalization for extensive-form games with general convex strategy constraints that can cut across decision points.

==> text/mixing_experts.tex <==
\section{Application: Mixing Experts}\label{sec:convex recommendation}

As an application, we consider the following scenario: an agent, called the ``combiner'', has to weight $n$ recommendations coming from $n$ individual experts. Furthermore, the loss incurred by the combiner is the same weighted average of $n$ independent losses, one for each of the experts.

More formally, we have $(\cX_i, \cL)$-regret minimizers (the ``experts''), $i=1,\dots, n$. We want to construct a regret minimizer that operates over the $n$-dimensional simplex $\Delta^n$, representing the space of all convex combination weights for the experts, and that faces losses of the form
\[
  \ell^t: \Delta^n \ni (\lambda_1,\dots,\lambda_n) \mapsto \lambda_1 \ell^t_1(x_1^t) + \dots + \lambda_n \ell^t_n(x_n^t),
\]
where $x_i^t$ and $\ell^t_i$ are respectively the recommendation of and the loss incurred by the $i$-th expert at time $t$.

We define
{\footnotesize\[
  \regret\mu := \sum_{t=1}^T {\tilde\ell}_t(\mu^i) - \min_{{\hat\mu}\in\sympl{m}} \left\{\sum_{t=1}^T {\tilde\ell}_t({\hat\mu}) \right\},
\]}%
where
{\footnotesize\[
  {\tilde\ell}_t: \mu \mapsto \sum_{i=1}^m \mu^i \ell_t(x^i_t).
\]}

Hence, 
{\footnotesize\begin{align*}
  \regret{\cX'} &= \sum_{t=1}^T \sum_{i=1}^m \mu^i_t \ell_t^i(x^1_t) - \min_{\substack{\hat\mu \in \sympl{m}\\\{{\hat x}^i \in \cX^i\}}} \left\{\sum_{t=1}^T \sum_{i=1}^m {\hat\mu}^i \ell_t^i({\hat x}^i)\right\}\\
    &= \sum_{t=1}^T \sum_{i=1}^m \mu^i_t \ell^i_t(x^i_t) - \min_{\hat\mu \in \sympl{m}} \left\{ \sum_{i=1}^m {\hat\mu}^i \min_{{\hat x}^i\in\cX^i} \left\{\sum_{t=1}^T\ell_t^i({\hat x}^i)\right\} \right\}\\
    &= \sum_{t=1}^T \sum_{i=1}^m \mu^i_t \ell^i_t(x^i_t) - \min_{\hat\mu \in \sympl{m}} \left\{ \sum_{i=1}^m {\hat\mu}^i \left(-\regret{\cX^i} + \sum_{t=1}^T\ell_t^i(x_t^i)\right) \right\}\\
    &\le \max_i \left\{\regret{\cX^i}\right\} + \regret{\mu}.
\end{align*}}

